Exploring and Adapting Chinese GPT to Pinyin Input Method

While GPT has become the de-facto method for text generation tasks, its application to pinyin input method remains unexplored. In this work, we make the first exploration to leverage Chinese GPT for pinyin input method. We find that a frozen GPT achieves state-of-the-art performance on perfect pinyin. However, the performance drops dramatically when the input includes abbreviated pinyin. A reason is that an abbreviated pinyin can be mapped to many perfect pinyin, which links to even larger number of Chinese characters. We mitigate this issue with two strategies, including enriching the context with pinyin and optimizing the training process to help distinguish homophones. To further facilitate the evaluation of pinyin input method, we create a dataset consisting of 270K instances from 15 domains. Results show that our approach improves performance on abbreviated pinyin across all domains. Model analysis demonstrates that both strategies contribute to the performance boost.

==> frozen-gpt.tex <==
\section{Language GPT}
\label{sec:frozen}

In this section, we first introduce the public GPT and then describe our further trained GPT.
% GPT2 further shows its generality in zero-shot settings over a wide range of tasks.

\subsection{GPT in the public}
GPT~\cite{radford2018improving,radford2019language} is a multi-layer transformer decoder pretrained over a large amount of data.
It shows strong ability in natural language inference, question answering, semantic similarity, and text classification. 

For applying GPT to address Chinese NLP tasks, the Chinese Pretrained Language Model (CPM) with 2.6 billion parameters, which is \citep{cpm-v1} trained on 100GB Chinese training data, has demonstrated strong performance. However, CPM is not a character-level model and is not applicable for pinyin input method. We turn to employ a widely adopted GPT2-Chinese~\cite{GPT2-Chinese} as our starting model. CPT2-Chinese is trained on 14GB Chinese training data CLUECorpusSmall~\cite{CLUECorpus2020}, which collected from Chinese news, Wikipedia, on-line forum message, and Consumer comments.
% In this section, we explore how GPT trained over Chinese corpus can be used to the PTC task.
% A straightforward approach is that we pass the user-confirmed context to GPT-2 as input, and we filter the predicted token distribution by keeping only those tokens whose Pinyin matches the target Pinyin syllable.

% To facilitate with evaluation using MIU, we adopt two commonly used corpora The People’s Daily corpus and TouchPal corpus~\cite{zhang-etal-arxiv-tracing}.


\subsection{Our GPT} 
To construct strong baselines, we further trained two kinds of GPT with 6 layers and 12 layers based on 800GB Chinese training data, which consists of news, Wikipedia, and novel texts. The configuration of 12-layer GPT is same as the standard GPT.\footnote{\url{https://huggingface.co/gpt2}} The 6-layer GPT is directly truncated and initialized from the converged 12-layer GPT and is continually trained. We train our 12-layer GPT with a batchsize of 2560 on 32x Tesla V100 GPUs. We adopt the Adam optimizer~\cite{kingma2014adam} and set the learning rate to 1e-5 with a linear warmup scheduler. We run the warmup process for 10k steps and train 100k steps in total. For 6-layer GPT, we train it for 50k steps with the same configuration of 12-layer GPT.

% \paragraph{GPT as a pinyin IME} To customize GPT2 for the task PTC, we need to use the pinyin sequence as a constraint during decoding.
% Given the mapping of pinyin syllables and their candidate characters, we can choose to decode characters from that specific syllable for each step.

% To test to what extent that GPT2 can do over the PTC task, we conduct the following experiments: 
% (1) we use CPM-Distill~\cite{cpm-v1} to do the pinyin-constrained decoding for comparison since it has the similar model size with our pretrained GPT,
% (2) we conduct the pinyin-constrained decoding on our pretrained GPT without finetuning on the PD dataset,
% (3) we finetune our pretrained GPT over PD dataset report evaluation results using differnt beam sizes.

% The detailed comparison of our experiments and related works are listed in Table~\ref{tab:miu} of Section~\ref{sec:pd}.
% The main conclusion we can draw is that a frozen GPT can achieve state of the art performance over the PTC benchmark if perfect pinyin is used as constraints during decoding.

==> pinyingpt.tex <==
\section{PinyinGPT}

\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{PinyinGPT.pdf}
\caption{Model.} 
\label{fig:pinyingpt}
\end{figure*}

% From Section~\ref{sec:frozen}, we know that plain GPT is already powerful over the PTC task with constrained decoding using perfect pinyin syllables.
% However, there's an increasing trend that users prefer to type abbreviations of pinyin.
% Suppose we use pinyin abbreviations rather than perfect syllables as the pinyin input, can GPT still achieve impressive performance?
% % To make pinyin IME more effective and efficient, typing shorter pinyin is a demand from users' perspective.
% % pinyin abbreviations have been investigated as inperfect input in some research~\cite{huang-etal-2018-moon}.
% % In consistent with them, we also define abbreviations of pinyin as the first character of each syllable.
% The answer is negative as our test shows that there will be a drastic drop in accuracy for all top-$K$, see Section~\ref{sec:abbr}.

In this section, we explore incorporating pinyin information into GPT to further strengthen its ability in the pinyin input method task, especially in the setting that the pinyin sequence contains only abbreviations.
We build two main kinds of models to inject the pinyin information:
(1) \textbf{Composition}: the idea of composition is to compose the token information of a specific token with the pinyin information of the next token.
(2) \textbf{Concatenation}: to make GPT aware of the \textit{whole} pinyin inputs, we concatenate the pinyin input sequence with the context input sequence to form a longer sequence before encoding using GPT.

\subsection{Composition} 

Depending on at which layer we inject the pinyin information, there are several variations of composition schemes for us to choose:
(1) \textbf{Bottom}: we can add the pinyin embedded information directly to the token embeddings at the bottom embedding layer before feeding the embeddings into GPT's encoder,
(2) \textbf{Top}: we can first compute the next token's distribution directly from the pinyin embedded information through a feed-forward layer and then add to the logits computed from original GPT.
% (3) \textbf{Stack}: we may also stack more transformer layers over GPT to better fuse the information of both tokens and pinyin.

For \textbf{Composition} models , we are given a text sequence $\mathbf{x} = [w_0,\dots,w_{T-1}]$, $w_0$ is the special start token \texttt{[CLS]} used in GPT, and a pinyin sequence $\mathbf{y} = [p_1,\dots,p_T]$ and perform finetuning over GPT by maximizing the following:
\begin{equation}
    \max_{\theta} \log p_{\theta}(\mathbf{x}) = \sum_{t=1}^{T-1}\log p_{\theta}(x_t|\mathbf{x}_{<t},\mathbf{y}_{<t})
\end{equation}

\subsection{Concatenation} 
The concatenation model takes the \textit{whole} pinyin sequence as part of its inputs. 
During training stage, the target character sequence will be further appended to the input sequence to calculate the autoregressive language model loss.
During inference stage, the generation starts conditioned over the context sequence and the pinyin sequence.
In practice, we expand the vocabulary of GPT $\mathcal{V}$ with the legitimate pinyin vocabulary $\mathcal{P}$, and use the special token \texttt{[SEP]} to separate the input text sequence and the pinyin sequence.
We are given an input sequence $\mathbf{x} = [w_0,\dots,w_l,\texttt{[SEP]},p_{l+1},\dots,p_{l+k},\texttt{[SEP]},w_{l+1},\allowbreak \dots,w_{l+T-1}]$.
To make the pinyin tokens to be aligned with the target tokens, we will share the positional embeddings of the pinyin token with its target token accordingly.
We perform finetuning over GPT by maximizing the following:
\begin{equation}
    \max_{\theta} \log p_{\theta}(\mathbf{x}) = \sum_{t=l+k}^{l + k+ T}\log p_{\theta}(x_t|\mathbf{x}_{<t})
\end{equation}

\subsection{Training}
\label{sec:training}

Unless specified explicitly, the corpus used for the training will be the same as that used when pretraining our own GPT.
Since the corpus is in pure text, we use a public library \textit{pypinyin}\footnote{\url{https://github.com/mozillazg/python-pinyin}} to get the pinyin of a piece of text.
Although the library is very helpful in labelling pinyin for most commonly used words, there are issues of heteronym for some characters which we further verified using online dictionaries like ZDic~(汉典)\footnote{\url{https://www.zdic.net/}}.

We start the training by initialize our model with a checkpoint from our pretrained Chinese GPT discussed in Section~\ref{sec:frozen}.

During training, we also changed the loss function to better suit the scenario of pinyin input method.
As pointed out in Section~\ref{sec:intro}, we choose to filter the predicted token distribution by keeping only those tokens whose pinyin matches the target pinyin syllable during generation.
Considering that the original loss of GPT is computed over the whole vocabulary, this leads to inconsistency between training and evaluation.
In this paper, we choose to use a modified loss function which focuses on the characters sharing the same pinyin.


Our models are trained using 32 GPUs of NVIDIA V100 Tensor Core with a bach size of 25,000 for 100k steps.
Our starting learning rate is set to be 5e-5 .
Each training case is sampled from the same corpus used for our pretraining of GPT.
We maintain a maximum of 128 tokens for every case.
When training the Concatenation model, we use a probability 0.5 to keep the target sequence to be less than 5 words, otherwise we randomly choose from a range 6 to 25 words.

